VideoWorld: Exploring Knowledge Learning from Unlabeled Videos

This work explores whether a deep generative model can learn complex knowledge solely from visual input, in contrast to the prevalent focus on text-based models like large language models (LLMs). We develop VideoWorld, an auto-regressive video generation model trained on unlabeled video data, and test its knowledge acquisition abilities in video-based Go and robotic control tasks. Our experiments reveal two key findings: (1) video-only training provides sufficient information for learning knowledge, including rules, reasoning and planning capabilities, and (2) the representation of visual change is crucial for knowledge acquisition. To improve both the efficiency and efficacy of this process, we introduce the Latent Dynamics Model (LDM) as a key component of VideoWorld. Remarkably, VideoWorld reaches a 5-dan professional level in the Video-GoBench with just a 300-million-parameter model, without relying on search algorithms or reward mechanisms typical in reinforcement learning. In robotic tasks, VideoWorld effectively learns diverse control operations and generalizes across environments, approaching the performance of oracle models in CALVIN and RLBench. This study opens new avenues for knowledge acquisition from visual data, with all code, data, and models open-sourced for further research.

==> sec/exp_old.tex <==


\section{Video-GoBench}
\label{sec:gobench}
Our goal is to explore whether a deep generative model can learn complex knowledge from raw videos, focusing especially on tasks requiring advanced planning and reasoning. We prioritize tasks that emphasize high-level planning and reasoning while minimizing dependence on low-level visual details like shape and texture.

%Our objective is to explore whether a deep generative model can learn complex knowledge. For better assessing the  especially in tasks that require sophisticated planning and reasoning. but are independent of low-level visual details like shape and texture. This approach allows us to assess the model's reasoning capabilities in a clear and focused manner. 
%In contrast, most real-world video data lacks the depth of complex knowledge and requires massive pre-training on internet-scale datasets to achieve high-quality generation,  introducing extra prior knowledge. Furthermore, the rich textures and motion in real-world videos can obscure the evaluation of a model's knowledge strength.
To this end, we introduce Video-GoBench, a purely visual Go benchmark, with a simple yet effective visual design to capture a broad range of complex knowledge and enable direct evaluation through online gameplay. By simplifying visuals, we minimize distractions from intricate textures and dynamics, allowing us to focus solely on assessing reasoning and planning ability. Additionally, the simulated Go environment allows for the seamless conversion of large-scale, state-based gameplay data into video sequences, supporting efficient and scalable evaluation.

\subsection{Dataset Generation}
To construct Video-GoBench, we collect 10 million 9x9 Go game records, including 3.2 million self-play training examples from  KataGo~\cite{wu2019katago} and 7.8 million from human-match games from OGS~\cite{ogs2024}. For the human data, we re-annotate the moves based on the original board states using KataGo to provide the optimal next moves for each state. The dataset comprises about 400 million unique board states, each converted into 256-pixel images. Additionally, we curated a test set of 1,000 matches, with each move re-annotated by KataGo. To enhance the test set’s ability to benchmark model generalization on new boards, we removed opening moves\textemdash given the limited diversity in early-game positions\textemdash resulting in 56,000 unique board states.


\subsection{Evaluation}
\label{subsec:goeva}
We use the following metrics to evaluate our models:
% on various levels of knowledge learning and   measure training progress:

\begin{itemize}
    \item   \textbf{Legal rate}: The percentage of legal moves generated by the model on the test set, indicating the model’s ability to understand and adhere to the basic rules of Go.

   \item  \textbf{Game playing strength (Elo)}: Following \cite{ruoss2024chessbench}, we evaluate models through an internal tournament. Eight agents, as shown in Tab.~\ref{table:videogo}, play 400 games per pair, totaling 11.2K games. Elo ratings are calculated using BayesElo~\cite{coulom2008elo} with a default confidence of 0.5. Among the agents are three versions of the KataGo engine, fine-tuned to 1-dan, 5-dan, and 9-dan human skill levels, to showcase the model’s strategic levels in relation to human play. We anchor the KataGo 9-dan model’s Elo rating at 2700, aligning with the standard human 9-dan score.

   \item  \textbf{Action accuracy}: Percentage of test instances where the model selects the best move made by KataGO (oracle).

   \item \textbf{Action-Value}: During tournament matches, we record the board state at each move and use KataGo-9d to annotate the action-values, which are the expected cumulative rewards for all possible moves in each state, serving as a value oracle. We then calculate the ratio of the action-value for each move made by the model to the optimal action-value. This metric measures the model's ability to evaluate moves. An action-value of 100\% indicates that the model's move matches the level of KataGo-9d.
\end{itemize}

% \vspace{-8em}
\section{Experiment}
\label{sec:experiment}
% In this section, we first introduce the implementation details. We then analyze the key observations we find in experiments and demonstrate the superior performance of VideoWorld by comparing with strong baselines.  Finally, we ablate on the key components in VideoWorld.

\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/umap_test_v5.png}
\centering
\vspace{-2em}
\caption{\textbf{Illustration of playing against KataGO} and UMAP projection~\cite{leland2018umap} of the predicted latent code. Our model plays as black. The generated latent code is visualized through the LDM decoder and new stones in the visualization are marked with colors to match the legend. The visualization serves as a probe, indicating that the model shows signs of forward planning.   }
\label{fig:umap_test}
\vspace{-1.5em}
\end{figure}
\input{tables/videogo}
\input{tables/calvin}
\input{tables/calvin_and_rlbench}
\input{tables/all_ablation_old}
% \input{tables/supp_abla}

\subsection{Implementation Details}
% \textcolor{red}{[JS: this paragraph is overlapped with the 'basic framework' section.]}
% Both the latent dynamics model and the auto-regressive Transformer encoder-decoder utilize the MAGVIT-v2 architecture \textcolor{red}{[JS: add reference]}, with temporal downsampling removed. For quantization, we employ the state-of-the-art FSQ~\cite{mentzer2024fsq} method as the quantizer, with a default vocabulary size of 64,000 tokens.
Our auto-regressive transformer is randomly initialized, with its encoder initially trained on the target dataset for reconstruction and then frozen. Trainable parameters including the transformer layers, projection layers, and output layers. The default vocabulary size for both LDM and transformer encoders is 64,000, corresponding to FSQ levels $[8,8,8,5,5,5]$.
For Go and CALVIN environments, we increase the number of downsampling layers in each encoder, compressing each frame to 4x4. We use a frame length of 6 for Go and 10 for CALVIN. We train and test in the CALVIN ABCD$\rightarrow$D split. RLBench shares the same training settings as CALVIN, with 20k trajectorie data generated by custom scripts. The training uses the AdamW~\cite{loshchilov2019adamw} optimizer with a learning rate of 0.0003 and no weight decay. The batch size is set to 256 for Go and 32 for CALVIN, requiring approximately 4 and 2 days of training on 8 A100 GPUs, respectively.

\subsection{Benchmarks}
We evaluate VideoWorld on three benchmarks: Video-GoBench, CALVIN and RLBench. Go tests long-horizon reasoning and complex forward planning, while last two focuses on more intricate visual changes.
For Go, we use the evaluation metric detailed in Sec.~\ref{subsec:goeva}. In CALVIN benchmark, our model controls a Franka Emika Panda robot with a parallel-jaw gripper in an environment with a desk, openable drawer, colored blocks, and an LED and light bulb. We evaluate three tasks: Push Blocks, Open/Close Drawer, and Turn On/Off Light. Each task is specified by an instruction label, such as ``{\tt go push the red block right}'',  which is provided to the transformer as a condition for video generation. In RLBench benchmark, the model controls the same robotic arm, but the environment and camera views differ from CALVIN. We evaluate two tasks: Close Microwave and Close Fridge. Object positions in both environments are randomly generated for each execution. We sample 500 tasks randomly and record the success rate.
%We evaluate VideoWorld on two benchmarks with different targets: Video-GoBench and the CALVIN Benchmark. Video-GoBench tests the model in scenarios requiring long-horizon reasoning and complex forward planning. The CALVIN benchmark, on the other hand, focuses on effectiveness in environments with more intricate visual changes. 


\subsection{Key Findings with The Basic Framework} 
\label{subsec:findings}

% \vspace{-15mm}
\noindent \textbf{Model can learn basic knowledge from raw videos.} As shown in Tab.~\ref{table:videogo} (idx 5) and Tab.~\ref{table:calvin} (line two), using the basic framework to train on Go videos and robotic videos enables the model to master the rules of Go, and learn basic robotic operation skills. On the Go test set, the model demonstrates almost 100\% legality, indicating that it has mastered rules including prohibitions against repeated moves, suicide moves, and more advanced rules like ko fights. Additionally, it achieves nearly a 50\% accuracy rate in predicting the best moves, showing a moderate understanding of Go strategy. In robotic scenarios, the model also demonstrates a certain ability to complete tasks. Compared to Go, handling more complex appearance without relying on pre-training imposes higher demands on the model's generation quality.



\noindent \textbf{Representation compactness is essential.} While the basic framework can learn knowledge from video, we find that using more compact representations leads to significantly better performance and efficiency. In Go, the state sequence, which includes the annotated position of each move is both information-rich and highly compact. In Tab.~\ref{table:videogo}, using these state sequences for training (idx 4) significantly improves performance on all metrics with the same amount of data. Fig.~\ref{fig:fig1} shows this clearly, with the state representation converging faster as training progresses. In robotic scenarios, although it is not feasible to fully represent the environment with state sequences, incorporating action labels for each frame also significantly boosts task completion rates. 

\subsection{Results with LDM} 
\label{subsec:res_ldm}
Based on the above observations, we introduce the Latent Dynamics Model (LDM) to enhance the efficiency and effectiveness of video learning, resulting VideoWorld model.

\noindent \textbf{Results on Go.}
In Tab.~\ref{table:videogo}, we compare VideoWorld with three official KataGo models calibrated to human skill levels: 1-dan, 5-dan, and 9-dan. The 1-dan model represents players with a foundational understanding of Go, while the 5-dan and 9-dan levels indicate progressively advanced skills, with 9-dan serving as an Oracle at the highest human level. Notably, all these models are RL-based, using search and reward mechanisms.

We evaluate VideoWorld at three parameter scales: 50M, 150M, and 300M. All models show strong generalization on novel boards. Even the smallest model, VideoWorld-50M surpasses KataGo-1d (Elo 2093 vs. 2019), while VideoWorld-300M outperforms the human-level KataGo-5d (Elo 2317 vs. 2253), demonstrating VideoWorld’s strong capability for mastering complex tasks. Compared to its counterpart without LDM, VideoWorld shows a significant improvement (Elo 2317 vs. 1998), underscoring the benefits of learning with latent representations.

Furthermore, we observe that performance across all metrics improves consistently with model size, suggesting that VideoWorld’s knowledge learning capabilities continue to scale effectively, with potential for further enhancements as model size increases. 
% In Tab.~\ref{table:videogo}, we compare VideoWorld with three KataGo models that align with human skill levels: 1-dan, 5-dan, and 9-dan. The 1-dan level represents players who has undergone systematic learning and understands the rules and strategies of Go, while the 5-dan and 9-dan levels represent more advanced and professional skill levels. The weights of these models are provided by the official KataGo team, accurately representing the playing strength of humans at corresponding levels.  We evaluate VideoWorld with 50M, 150M, and 300M parameters. The results show that all three models generalize well to novel boards. VideoWorld also significantly narrows the gap mentioned in Sec.~\ref{subsec:findings}, achieving performance exceeding  that of a 5-dan human player. Across all metrics, increasing model size consistently leads to improved performance, underscoring the importance of model scale in learning complex knowledge from videos effectively.




\noindent {\textbf{Results on CALVIN.}} Tab.~\ref{table:calvin} presents the results of the models on the CALVIN benchmark. VideoWorld, relying solely on observed videos and does not use action labels, achieves performance close to that of models supervised with real action labels. This demonstrates that our proposed LDM effectively supports video-based knowledge learning, even in more visually complex scenarios. Furthermore, we use a supervised learning agent~\cite{wu2023gr1} to generate an additional 30k trajectory data in the CALVIN environment, which we incorporate into VideoWorld's training. As shown in Tab.~\ref{table:calvin}, VideoWorld demonstrates data scaling capabilities, further approaching oracle performance as data volume increases. This demonstrates the potential of our method for application in larger-scale training.


\noindent {\textbf{Generalization across multiple environments.}} To further validate VideoWorld's generalization across different environments, we introduce two additional tasks from RLBench, which are visually distinct from CALVIN: closing microwave and closing fridge. For each task, we generate 10k trajectories and train VideoWorld on this data combined with CALVIN. We then evaluate task success rate in both environments. As shown in Tab.~\ref{table:calvinrlbench}, VideoWorld generalizes well across two settings, simultaneously mastering skills in two environments and approaching the performance of the oracle setup. Reinforcement learning methods often struggle to generalize across different environments, as they heavily rely on task-specific states/action/rewards, etc. This also demonstrates the potential of our method to serve as a general knowledge learner. See Supp.~\ref{sec:supp_detail} for more detail.
% To our best knowledge, VideoWorld is the first to explore learning complex knowledge solely through video generation. To demonstrate its effectiveness, we compare with the following strong reinforcement learning (RL) based baselines and supervised learning (SL) baselines. 
% \begin{itemize}
% \item \textbf{Reinforcement Learning Go Agents}: With the ability to iteratively improve through explicit search and self-play, RL agents have significant advantages over supervised learning in board games, achieving superhuman performance. Our aim is not to surpass the most advanced reinforcement learning AI but to validate that video-based supervised learning can acquire similar strategies. Therefore, we choose KataGo models that align with human skill levels:1-dan, 5-dan, and 9-dan. The 1-dan level represents players who has undergone systematic learning and understands the rules and strategies of Go, while the 5-dan and 9-dan levels represent more advanced and professional skill levels. The weights of these models are provided by the official KataGo team, accurately representing the playing strength of humans at corresponding levels.  
% \item \textbf{Supervised Learning Go Agents}: We select a model trained with Behavior Cloning using Go state sequences, representing an oracle setting where all environmental information is compactly encapsulated in the state. Additionally, we include a model trained with pure video-based Behavior Cloning that does not utilize the LDM.
% \item \textbf{Supervised Learning Robotics Agents}: Given the higher visual complexity of robotic scenarios, the oracle setting that relies solely on state information is infeasible. Therefore, we train a baseline model that takes images as input and outputs real action labels for supervision. Additionally, we train a model that bypasses the LDM, using an inverse dynamics model to convert generated video frames into executable actions.
% \end{itemize}

% Tab.~\ref{table:videogo} compares VideoWorld with competing methods on the Video-GoBench. 
% We evaluate models with 50M, 150M, and 300M parameters. The results show that all three models generalize well to novel boards and can  predict a substantial fraction of the best moves. The extremely low rate of illegal moves indicates that the models have mastered the fundamental rules of Go, including prohibitions against repeated moves, self-capture, and more advanced rules like ko fights. 

% In tournament matches, models trained directly on video also achieves strong action values, reaching a level comparable to that of a 1-dan human player. However,   there remains a notable gap compared to the models trained from a more compact state space representation. Our approach \textcolor{red}{[JS: what approach]} significantly narrows this  gap, achieving performance exceeding   that of a 5-dan human player. Across all metrics, increasing model size consistently leads to improved performance, underscoring the importance of model scale in learning complex knowledge from videos effectively.

% \subsection{Results on CALVIN} 
% Tab.~\ref{table:calvin} presents the results of the models on the CALVIN benchmark. VideoWorld, relying solely on observed videos and does not use action labels, achieves performance close to that of models supervised with real action labels. This demonstrates that our proposed LDM effectively supports video-based knowledge learning, even  in more visually complex scenarios. 

% Notably, when LDM is omitted, the task success rate drops significantly. This decline is closely tied to the lack of publicly available, high-quality pre-trained models for video next token prediction. Figure X shows some generated samples from the models. While the videos generated without LDM exhibit correct rough motion, the poor generation quality severely hampers the precision of action conversion. Incorporating LDM not only improves   the quality of the generated video but also enhances the efficiency of strategy learning \textcolor{red}{[JS: which results evidience the learning efficiency is improved?]}, acting as a guide for better video generation.

\subsection{Understanding Learned Knowledge with LDM}
The latent representation learned in LDM provides valuable insights into the knowledge learning process of VideoWorld. Below we offer an in-depth analysis of what our model learns through latent representations.
% \begin{enumerate} 

\noindent {\textbf{LDM learns patterns in the training set.}} As shown in Fig.~\ref{fig:umap}, the latent codes on the training set capture both short- and long-term dependencies, demonstrating the model's ability to represent knowledge at different temporal scales. In the Go scenario, salient regions in the latent codes correspond to common move patterns, indicating that the model effectively embeds multi-step strategies into a compressed space, hence aiding decision-making and reasoning. Similarly, in the robotics scenario, the clustering of latent codes across steps reveals key dynamic dependencies over various time ranges, thus benefiting diverse manipulation tasks.

\noindent {\textbf{LDM enables forward planning during testing.}} We examine the role of latent codes during inference. The visualization in Fig.~\ref{fig:umap_test} shows that codes from different steps group by output positions, suggesting that VideoWorld models long-range changes progressively, similar to human forward-planning. The visualization also includes imagination of the opponent's moves, achieving a high average action-value of 71.2\% and action accuracy of 74.3\%. This indicates that, at each step, VideoWorld considers long-term changes in the game situation within the latent space, enabling it to make strategic moves with a long-term perspective. Supp.~\ref{subsec:code_ana} shows a similar pattern in robotic scenario.

\noindent {\textbf{LDM generates causally interrelated codes.}} To further investigate the impact of the learned latent codes, we conduct an intervention experiment in Tab.~\ref{tab:abla_intervene}. We replace latent codes at different time steps with random tokens and observe the effect on performance. Intervening with the first code has the greatest effect, likely due to the causal dependencies learned among the codes. This aligns with intuition: altering the first code, which represents the immediate next optimal decision, affects all future decisions over a longer horizon. These results highlight the importance of the order and structure of latent codes for effective reasoning.


% \end{enumerate}
% \begin{enumerate}
%     \item As shown in Fig.~\ref{fig:umap},  the latent codes on training set   capture both short-term and long-term dependencies, revealing how the model learns to represent knowledge at various temporal scales. For Go, LDM models multi-step board changes, implicitly embedding long-term planning into the codes. For robotics, LDM can capture displacement changes over various time spans.
%     \item During testing, Fig.~\ref{fig:umap_test} shows how the model mimics human forward-planing strategies, accounting for long-term changes in the battle situation within a high-dimensional space. This enables VideoWorld to comprehensively evaluate the current state and make the most strategic move over the long run. Examples of the codes when performing robotic tasks are provided in Supp.
%     \item We also conduct an intervene experiment in Tab.~\ref{tab:abla_intervene} to further investigate the effect of the learned latent codes We replace latent codes at different time-step with random tokens and observe the effects on performance. We find that intervening with the first code has the greatest impact. This is likely because the latent codes in LDM training reconstruct the video sequence causally, creating dependencies between the codes.highlighting that the ordering and structure of the latent codes are critical for enabling  the model to think and reason effectively.
% \end{enumerate}



\subsection{More Ablations}

\noindent \textbf{Horizon length in latent dynamics model.} Tab.~\ref{tab:abla_timespan} shows the effects of varying compression lengths during LDM training. 
We use a default compression length of 5 steps for Go and 10 steps for CALVIN.
% For Go, we use a default compression length of 5 steps, and for CALVIN, we use 10 steps.
When we vary the compression length while keeping the codebook size constant, we observe that with a compression length of 1 step (similar to pseudo action labels), both Go and CALVIN improvement significantly over the baseline. For Go, optimal performance is at 5 steps, but further increasing the length causes the LDM training to fail to converge. We attribute this to the exponential growth in possible board position variations, which overwhelms the codebook and causes training instability. In contrast, the simpler dynamic changes in CALVIN environment allow for longer compression lengths.

% \noindent \textbf{Intervene latent visual process codes.} 

\noindent \textbf{Latent codebook size.}    Tab.~\ref{tab:abla_codebooksize} examines the impact of LDM's codebook size on knowledge learning. By adjusting the FSQ level, we test four different codebook sizes to evaluate how this affects the model's ability to learn effective policies. In the Go scenario, we find that even a smaller vocabulary yields significant improvements; however, this is not the case for the robotic scenario. This discrepancy likely arises because the robotic scenario involves more motion and appearance information, requiring a larger vocabulary to capture essential details. When the vocabulary size becomes too large, LDM training struggles to converge, leading to a noticeable performance drop in both scenarios.

% \noindent \textbf{Latent code prediction only.}
% To demonstrate the necessity of  jointly predicting the latent code $\{\hat{z}_t^h\}_{h=1}^H$ and next frame $\hat{x}_{t+1}$ given $x_{1:t}$, we remove the supervision for the next frame $\hat{x}_{t+1}$ during training. In this setup, frames are only used as input, and only the latent codes are subject to the CE loss. In this case, we retrain an IDM that only receives latent code inputs.
% As shown in Tab.~\ref{table:supp_onlylc_go}, for both Go and robotic scenarios, using codes alone significantly improves performance, and incorporating next-frame prediction further enhances it. We hypothesize this is because next-frame prediction enhances the model's understanding of the environment and helps generate more accurate codes.

%because Go moves are simple, and a smaller vocabulary can still capture the necessary information. In contrast, the robotic scenario requires precise continuous actions, demanding a larger vocabulary. 
%When the vocabulary size increases too much, LDM training struggles to converge, resulting in a noticeable performance drop in both scenarios.

\noindent \textbf{Data quality.} Tab.~\ref{tab:abla_data} examines the effect of data quality on learning. Video-GoBench dataset has two types of data: human matches and KataGO self-play matches. These data sources have different distributions, and their policy content varies, potentially influencing the learning process. We find that using the original human data significantly impacts the final performance, as it includes players of varying skill levels, highlighting the importance of data quality.
 
% \noindent \textbf{Data quality}
% 

\vspace{-1mm}
\section{Conclusion}
\label{sec:discusion}

In this work, we take an initial step toward exploring knowledge learning from raw video data using the next token prediction paradigm. We conduct systematic experiments in custom Video Go and robotic simulation environments. We present two key findings: \textit{i}) The model can master the rules of Go and learn fundamental robotic operations, and \textit{ii}) The compactness of visual representation is crucial for efficient knowledge learning. Based on these findings, we propose a latent dynamics model (LDM) to enhance the efficiency of knowledge learning. Although applying this approach to real-world scenarios still faces challenges such as high-quality video generation and generalization, we believe that video generation models have the potential to serve as general knowledge learners and ultimately function as the artificial brain capable of thinking and acting in the real world.




==> sec/supp_old.tex <==
\clearpage
\newpage
\appendix
\setcounter{page}{1}
\maketitlesupplementary

% \clearpage
% \setcounter{page}{1}
% \maketitlesupplementary
% \appendix

\renewcommand\thefigure{\thesection.\arabic{figure}}
\renewcommand\thetable{\thesection.\arabic{table}}
\setcounter{figure}{0} 
\setcounter{table}{0} 
\setcounter{table}{0}
\renewcommand{\thetable}{A.\arabic{table}}

% In this supplementary material, we first detail the training configuration, latent dynamics model, robotics action execution and inverse dynamics model in Sec.~\ref{sec:supp_detail}. Next, we present further analysis of latent dynamics model in Sec.~\ref{sec:supp_abla}. We also offer a comprehensive analysis of Video-GoBench in Sec.~\ref{sec:supp_dataset} and include more visualization results in Sec.~\ref{sec:supp_vis}.

% In this supplementary material, we first detail the training configurations, the latent dynamics model, robotics action execution and the inverse dynamics model in Sec.~\ref{sec:supp_detail}. Next, we present further analysis of the latent dynamics model in Sec.~\ref{sec:supp_abla}. We also offer a comprehensive analysis of Video-GoBench in Sec.~\ref{sec:supp_dataset} and include more visualization results in Sec.~\ref{sec:supp_vis}.

In this supplementary material, we first detail the training configurations, the latent dynamics model, robotics action execution, and the inverse dynamics model in Sec.~\ref{sec:supp_detail}. Next, we present further analysis of the latent dynamics model in Sec.~\ref{sec:supp_abla}. We also offer a comprehensive analysis of Video-GoBench in Sec.~\ref{sec:supp_dataset} and include additional visualization results in Sec.~\ref{sec:supp_vis}.

\section{Implementation Details}
\label{sec:supp_detail}

\noindent \textbf{Training details.} We present the detailed training configurations of latent dynamics model and auto-regressive transformer in Tab.~\ref{table:supp_training_setting}.

\noindent \textbf{Latent dynamics model.}  The decoder can be divided into three parts based on three functions: \textit{i}) using an encoder to causally extract image features; \textit{ii}) using learnable embeddings to extract change information from the extracted features; \textit{iii}) using a decoder to causally reconstruct video frames based on image feature of the initial frame and the learned embeddings. We present the PyTorch-style pseudocodes for the overall LDM and each part in Alg.~\ref{alg:code}.

\noindent \textbf{Robotics action execution.}
Our model generates a set of latent codes $\{\hat{z}_t^h\}_{h=1}^H$ and next frame prediction $\hat{x}_{t+1}$ based on language instruction and input sequence $x_{1:t}$. We feed $\{\hat{z}_t^h\}_{h=1}^H$, $\hat{x}_{t+1}$ and $x_t$ into the Inverse Dynamics Model to obtain corresponding action. The inferred action is executed in an open-loop manner: after predicting each action, we input it into the environment engine to obtain a new observation $x_{t+1}$, which is then appended to the input sequence for the next prediction cycle. In Fig.~\ref{fig:umap_test_calvin}, we visualize the model's next-frame predictions and the actual control results of the robotic arm. We find that the model's next-frame predictions align with the task's execution intent and effectively control the robotic arm to complete the tasks. We also visualize the latent codes at different time steps during testing and analyze them in Sec.~\ref{subsec:code_ana}.

\noindent \textbf{Inverse dynamics model.}
% The training objective of IDM is to directly predict the control signals for the robotic arm, a 7-dimensional vector that includes the arm's displacement along the XYZ axes, Euler angles, and the gripper's open/close state. Our IDM uses a ResNet-18 with an avgpool layer to process the mean squared error between two frames, resulting in a feature vector of size (1, 512). Simultaneously, IDM uses an MLP to process the latent codes' corresponding feature vectors into size ($H$, 512), $H$ is defined in Sec.3.2 and represents the total number of learnable embeddings in the LDM. Finally, another MLP with dimensions (512, 7) and an avgpool layer processes this ($H$+1, 512) vector into the final control signals.
% IDM is trained using the AdamW optimizer with a learning rate of 1e-4 for a total of 1M steps.
%The training objective of IDM is to directly predict the control signals for the robotic arm, which is a 7-dimensional vector including the arm's displacement along the XYZ axes, Euler angles, and the gripper's open/close state. Our IDM uses a ResNet-18 with an avgpool layer to process the frames to compute the mean squared error, resulting in a feature map and then avgpool it to size (1, 512). Simultaneously, the IDM uses an MLP to process the latent codes' corresponding feature vectors into a feature vector of size ($H$, 512). $H$ is defined in Section 3.2 and represents the total number of learnable embeddings in the LDM. Finally, another MLP with dimensions (512, 7) and an avgpool layer processes this vector of size ($H$+1, 512) into the final control signals.
The training objective of IDM is to predict the control signals for the robotic arm, represented as a 7-dimensional vector that includes the arm's displacement along the XYZ axes, Euler angles, and the gripper's open/close state. Specifically, IDM uses a ResNet-18 to process the predicted frame, applying a global average pooling layer to the penultimate feature map to obtain a feature vector of size (1, 512). Simultaneously, a shared MLP transforms the feature vectors of each latent code into a size of ($H$, 512), where $H$, as defined in Sec. 3.2, represents the number of learnable embeddings or prediction steps in LDM. Then, the features from the latent codes and the generated frames are concatenated into a vector of size ($H+1$, 512), which is then passed through another MLP with dimensions (512, 7) followed by a global average pooling layer to produce the final 7 control signals. IDM is trained using AdamW with a learning rate of 1e-4 for a total of 1 million steps, with mean squared error as the objective.

\noindent \textbf{RLBench evaluation.} In Sec.~\ref{subsec:res_ldm}, we test VideoWorld's ability to perform tasks in two different environments: CALVIN and RLBench. For CALVIN, we maintain the original task settings. For RLBench, we generate 20k trajectory data using a script. RLBench uses the same robotic arm and action space as CALVIN, but the environment appearance and task settings differ significantly. We use the combined RLBench and CALVIN datasets to train both the LDM and Transformer, while IDM is trained separately in each environment. Fig.~\ref{fig:supp_vis_rlbench} shows VideoWorld performing robotic tasks in RLBench environment.  

\input{tables/supp_detail}
% \input{tables/supp_baseline}
% \input{tables/supp_abla}
\section{Extended Analysis and Ablative Studies}
\label{sec:supp_abla}


\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/umap_calvin.png}
\centering
% \vspace{-2em}
\caption{\textbf{Illustration of robotic manipulation} and UMAP projection of the predicted latent code during inference. Latent codes are visualized through the LDM decoder. The UMAP projection illustrates the 9 predicted latent codes (i.e. $H=9$) across different tasks, with each point color-coded by task type. Visualizations with a yellow background show the model's actual robotic arm control during inference, while those with a green background represent the model's next-frame predictions during training.}
\label{fig:umap_test_calvin}
\vspace{-1.5em}
\end{figure}

\input{tables/ldm_alg}



\subsection{Understanding Learned Knowledge with LDM}
\label{subsec:code_ana}
In Sec. 5.5 of the main text, we analyze the role of LDM in the Go scenario, showing that latent codes contain information about board changes and can model long-range changes progressively. Similar findings are observed in the robotics scenario. In Fig.\ref{fig:umap_test_calvin}, we visualize the predicted latent codes during inference across different tasks. Here, $H=9$, meaning the auto-regressive transformer generates 9 latent codes at each time step, corresponding to 9 prediction steps. As shown in Fig.\ref{fig:umap_test_calvin}, the latent codes for different prediction steps are grouped by the type of manipulation task, indicating that they capture task-relevant dynamic information. For codes corresponding to prediction steps 1–4, the grouping shows greater overlap, likely because these codes focus on fine-grained displacements shared across tasks. In contrast, as the prediction steps extend to 5–9, the separation by task type becomes more distinct, highlighting the model's ability to progressively capture long-range changes specific to each task.
% the distinction between clusters of latent codes for different tasks improves, demonstrating the model's ability to capture long-range changes progressively. 





% \subsection{Ablative Studies}
% \noindent \textbf{Baseline comparisons on CALVIN.}
% To comprehensively analyze our method's performance, we compared it with two supervised learning methods: MCIL~\cite{mees2022matterslanguageconditionedrobotic} and HULC~\cite{lynch2021languageconditionedimitationlearning}. Both use ground truth labels for supervision. As shown in Tab.~\ref{table:supp_calvin}, when using GT labels, our oracle model trained with the next-token prediction paradigm achieves the best results, highlighting the strength of this paradigm. Even without action labels, our VideoWorld performs on par with other baselines and surpasses MCIL in all three tasks.

% \noindent \textbf{Latent code prediction only.}
% To demonstrate the necessity of  jointly predicting the latent code $\{\hat{z}_t^h\}_{h=1}^H$ and next frame $\hat{x}_{t+1}$ given $x_{1:t}$, we remove the supervision for the next frame $\hat{x}_{t+1}$ during training. In this setup, video frames are only used as input, and only the latent codes are subject to the CE loss. In this case, we retrain an IDM that only receives latent code inputs.
% As shown in Tab.~\ref{table:supp_onlylc_go}, for both Go and robotic scenarios, using latent codes alone significantly improves performance, and incorporating next-frame prediction further enhances it. We hypothesize this is because next-frame prediction enhances the model's understanding of the environment and also helps generate more accurate latent codes.


\begin{figure}[t]\centering
  \subfloat[\label{fig:state_count}Distribution of  board state count in training set]{\includegraphics[width=\linewidth]{figures/state_count.png}  }\\
% \hfill
\subfloat[\label{fig:state_rep}Repetition rate during online battle.]{\includegraphics[width=\linewidth]{figures/rep.png} }
\hfill

\caption{\textbf{Dataset statistics}. Best viewed digitally.}
\vspace{-3mm}
\label{fig:supp_data}
\end{figure}

\begin{figure}[t]\centering
  \subfloat[\label{fig:supp_vis_cap}Capture opponent's stones]{\includegraphics[width=\linewidth]{figures/supp_vis_cap.png}  }\\
% \hfil
\vspace{-1em}
\subfloat[\label{fig:supp_vis_sac}Sacrificing short-term gains to capture more opponent stones.]{\includegraphics[width=\linewidth]{figures/supp_vis_sac.png} }
\hfill
\vspace{-0.5em}
\caption{\textbf{Visualizations of learned Go Strategies}. our model captures opponent stones using the squeeze tactic and self-sacrifice tactic. New black stones are red, new white stones are blue.}
% \vspace{-1em}
\label{fig:supp_vis_go}
\end{figure}


\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/supp_vis_calvin_3.png}
\centering
\vspace{-2em}
\caption{\textbf{Visualizations of performing CALVIN tasks.}}
\label{fig:supp_vis_calvin}
\vspace{-1em}
\end{figure}
% Visualizations of VideoWorld performing robotic manipulation task} in CALVIN environment.

\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/supp_vis_rlbench.png}
\centering
\vspace{-2em}
\caption{\textbf{Visualizations of performing RLBench tasks.}}
\label{fig:supp_vis_rlbench}
\vspace{-1.5em}
\end{figure}
% Visualizations of VideoWorld performing robotic manipulation task} in RLBench environment.

\section{Details on Video-GoBench}
\label{sec:supp_dataset}

% \subsection{Dataset Statistics}
In this section, we systematically analyze Video-GoBench. The benchmark includes many unique board states, offering extensive references for the model to learn from. Moreover, due to the combinatorial explosion effect, the proportion of repeated board states\textemdash those encountered during inference that also appear in the training set\textemdash decreases sharply as the game progresses when our model competes against reinforcement learning agents. This ensures that good performance cannot rely on memorizing training scenarios, highlighting the model’s generalization ability.

\noindent \textbf{Board state count.}
The Video-GoBench training set contains approximately 400M unique board states. We analyze their distribution based on move numbers, i.e., the number of stones each state contains. As shown in Fig.~\ref{fig:state_count}, the data features a diverse range of board states, primarily concentrated within the first 100 moves, with significantly fewer states beyond that.

\noindent \textbf{Board state repetition rate.}
We collect 400 game records between our model and KataGo-9d, calculating the overlap rate of board states with the training set across different move numbers. As shown in Fig.~\ref{fig:state_rep}, the repetition rate drops sharply as the games progress. By move 30, it reaches zero, with all games continuing beyond this point. This eliminates the possibility of relying on memory alone to achieve high performance.
% \begin{figure}[t]
% \includegraphics[width=\linewidth]{figures/supp_repetition_rate.png}
% \centering
% % \vspace{-2em}
% \caption{ }
% \label{fig:supp_repetition}
% \vspace{-1.5em}
% \end{figure}






\section{Additional Visualizations}
\label{sec:supp_vis}
We provide more visualizations of VideoWorld performing Go and robotic tasks in Fig.~\ref{fig:supp_vis_go} and Fig.~\ref{fig:supp_vis_calvin}, respectively. The Go visualizations are from matches between our 300M VideoWorld and KataGo-5d. With comparable Elo scores, these matches fairly demonstrate of how the model applies its learned knowledge. In Fig.~\ref{fig:supp_vis_cap}, our model captures opponent stones using the squeeze tactic. In Fig.~\ref{fig:supp_vis_sac}, VideoWorld deliberately sacrifices a single stone, prompting the opponent to capture it, thereby creating an opportunity to capture more of the opponent's stones. This highlights the model’s ability to prioritize long-term planning over short-term gains. For the robotic scenario, we show the model’s actual control results for the robotic arm, demonstrating its understanding of manipulation tasks and ability to execute them effectively.

==> tables/all_ablation.tex <==
\begin{table*}[t]
\centering
\vspace{-0.5em}
%#################################################
% MAE decoder depth
%#################################################
\subfloat[
Different Compression length on Go.
\label{tab:abla_timespan}
]{
\centering
\begin{minipage}{0.45\linewidth}{\begin{center}
\tablestyle{5pt}{1}
\begin{tabular}{c cc}
    % \toprule
    \multicolumn{1}{c|}{\multirow{2}*{\makecell{Compression \\ length $H$}}}  &\multicolumn{2}{c}{Go}    \\
      \multicolumn{1}{c|}{} &Act-Value & Act-Acc.   \\
    \shline
    \specialrule{0em}{0pt}{1pt}
    \multicolumn{1}{c|}{baseline} &47.5  &44.3 \\
    % baseline &31.8  &40.6  &55.1 &56.0\\
    % + Higher resolution &40.1  &47.2 &64.3 &65.6\\
    
    \multicolumn{1}{c|}{1} &70.3  &77.0  \\
    \multicolumn{1}{c|}{3} &\underline{72.5}  &\underline{80.6} \\
    % \hline
    \multicolumn{1}{c|}{5} &\textbf{73.9}  &\textbf{80.9} \\
    && \\
\end{tabular}
\vspace{-1em}
\end{center}}
\end{minipage}
}
\hspace{1em}
%#################################################
% MAE decoder width
%#################################################
\subfloat[
Different Compression length on CALVIN.
\label{tab:abla_timespan_calvin}
]{
\begin{minipage}{0.45\linewidth}{\begin{center}
\tablestyle{5pt}{1}
\begin{tabular}{c  ccc}
    % \toprule
    \multicolumn{1}{c|}{\multirow{2}*{\makecell{Compression \\ length $H$}}}  &\multicolumn{3}{c}{CALVIN}    \\
      \multicolumn{1}{c|}{} & Push & Open/Close &Turn On/Off   \\
    \shline
    \specialrule{0em}{0pt}{1pt}
    \multicolumn{1}{c|}{baseline} &12.7  &20.8 &15.6 \\
    % baseline &31.8  &40.6  &55.1 &56.0\\
    % + Higher resolution &40.1  &47.2 &64.3 &65.6\\
    
    \multicolumn{1}{c|}{1} &33.7  &53.6 &67.3  \\
    \multicolumn{1}{c|}{5} &\underline{46.8}  &\underline{66.1} &\underline{69.6} \\
    % \hline
    \multicolumn{1}{c|}{10} &\textbf{50.3}  &\textbf{71.1} &\textbf{69.7} \\
    &&& \\
\end{tabular}
\vspace{-1em}
\end{center}}
\end{minipage}
}
\hspace{1em}
%#################################################
% MAE with mask token on encoder
%#################################################
\\
\centering
\vspace{-1em}
%#################################################
% MAE targets
%#################################################
\subfloat[
Different codebook size of LDM.
\label{tab:abla_codebooksize}
]{
\begin{minipage}{0.49\linewidth}{\begin{center}
\tablestyle{5pt}{1}
 \begin{tabular}{ c | cc | ccc}
                % \toprule
                  \multirow{2}*{\makecell{LDM \\ codebook  size  }}  \multirow{2}*  & \multicolumn{2}{c|}{Go} &\multicolumn{3}{c}{CALVIN} \\
                 
                     &Act-Value  &Act-Acc. &Push  &Open/Close &Turn On/Off  \\
                \shline
                \specialrule{0em}{0pt}{1pt}
                  729 &65.5   &71.1 &12.9 &20.0 &16.0     \\
                   15,625&\underline{69.3}   &\underline{72.8} &20.5 &24.1 &\underline{36.3}    \\
                  64,000&\textbf{73.9}   &\textbf{80.9} &\textbf{50.3}  &\textbf{71.1} &\textbf{69.7}   \\
                  262,144&50.1  &53.2  &\underline{29.8} &\underline{30.0} &31.7 \\
                % 4 & \Checkmark & \Checkmark & \Checkmark & 52.9 & \textbf{54.0} \\
                % \bottomrule
            \end{tabular}
\end{center}}
\end{minipage}
}
\hspace{1em}
\subfloat[
Intervene latent codes with different index
\label{tab:abla_intervene}
]{
\begin{minipage}{0.45\linewidth}{\begin{center}
\tablestyle{5pt}{1}
\begin{tabular}{c | cc }
    % \toprule
     \multirow{1}*{\makecell{ Index}} &\multicolumn{2}{c}{Go}  \\
     &Act-Value  &Act-Acc.    \\
    \shline
    \specialrule{0em}{0pt}{1pt}
    None  &\textbf{73.9}  &\textbf{80.9}      \\
    1 &46.2  &42.1    \\

    2 &69.5  &76.6     \\
    
    3  &\underline{72.1}  &\underline{80.6}     \\
    All  &45.8  &43.7   \\
\end{tabular}
\end{center}}
\end{minipage}
}
\\

% %#################################################
% % MAE data aug
% %#################################################
% \subfloat[
% \textbf{Data augmentation}. Our MAE works with minimal or no augmentation.
% \label{tab:aug}
% ]{
% \centering
% \begin{minipage}{0.29\linewidth}{\begin{center}
% \tablestyle{4pt}{1.05}
% \begin{tabular}{y{54}x{22}x{22}}
% case & ft & lin \\
% \shline
% none & 84.0 & 65.7 \\
% crop, fixed size & 84.7 & 73.1 \\
% crop, rand size & \baseline{\textbf{84.9}} & \baseline{\textbf{73.5}} \\
% crop + color jit & 84.3 & 71.9 \\
% \end{tabular}
% \end{center}}
% \end{minipage}
% }
% \hspace{1em}
%#################################################
% MAE with mask types
%#################################################


\centering
\subfloat[
Latent code prediction only.
\label{tab:abla_code_only}
]{
\begin{minipage}{0.49\linewidth}{\begin{center}
\tablestyle{5pt}{1}


 \begin{tabular}{c|cc|ccc}
    % \toprule
    \multirow{2}*{\makecell{Prediction \\ Target}}    &\multicolumn{2}{c|}{Go} &\multicolumn{3}{c}{CALVIN}   \\
      &Act-Value & Act-Acc. &Push & Open/Close &Turn on/off   \\
    \shline
    \specialrule{0em}{0pt}{1pt}
    video &47.5 &44.3 &12.7  &20.8 &15.6 \\
    % baseline &31.8  &40.6  &55.1 &56.0\\
    % + Higher resolution &40.1  &47.2 &64.3 &65.6\\
    
    code &73.0  &78.6 &47.2 &70.0 &65.1 \\
    code/video &73.9  &80.9 &50.3 &71.1 &69.7 \\
    % \hline
    % \bottomrule           
\end{tabular}
\end{center}}
\end{minipage}
}
\subfloat[
Data source ablation. $^\dagger$ means human data without re-annotation.
\label{tab:abla_data}
]{
\begin{minipage}{0.45\linewidth}{\begin{center}
\tablestyle{5pt}{1}
\begin{tabular}{l | c|cc }
    % \toprule
    \multirow{2}*{\makecell{Data \\ source}} &\multirow{2}*{\makecell{Data \\amount}} &\multicolumn{2}{c}{Go}  \\
    &  & Act-Value & Act-Acc.  \\
    \shline
    \specialrule{0em}{0pt}{1pt}
    Human$^\dagger$ &6.8M &34.6 &34.8  \\
    Human &6.8M &\underline{71.5} &75.7  \\
    % \specialrule{0em}{0pt}{1pt}
            % \hline
            % \specialrule{0em}{0pt}{1pt}
    KataGo &3.2M &70.8 &\underline{77.5} \\
    
     
     All &10M &\textbf{73.9} &\textbf{80.9}  \\
\end{tabular}
\end{center}}
\end{minipage} 
}

%#################################################
\vspace{-0.5em}
\caption{\textbf{Ablations and analysis.} We conduct all experiments based on our 50M model.}
\label{tab:ablations} \vspace{-1.5em}
\end{table*}

==> tables/re_ablation.tex <==

\begin{table} \centering
\vspace{-1em}
\footnotesize
% \scalebox{0.78}{
\resizebox{\columnwidth}{!}{
\begin{tabular}{lp{0.8cm}c cc cc}
% \vspace{-1em}
% \toprule[1pt]
    Method  &Input &Push &Open/Close &Turn on/off &Consecutive \\
    % \midrule
    \specialrule{0em}{0pt}{1pt}
    \shline
    \specialrule{0em}{0pt}{1pt}
    SPIL \textcolor{cvprblue}{[\scriptsize{ICLR'24,} arxiv.org/abs/2305.19075]}  &Vid/Act &68.4&87.9&85.3&55.4 \\
    LCD \textcolor{cvprblue}{[\scriptsize{RA-L'24,} arxiv.org/abs/2210.15629]}
    &Vid/Act &71.3&90.2&92.1&60.7 \\
%    {\color{lightgray}Transformer (Oracle)} &{\color{lightgray}Vid/Act} &{\color{lightgray}75.4} &{\color{lightgray}95.3} &{\color{lightgray}96.2} &{\color{lightgray}68.0 }\\
    Transformer &Vid &17.3 &24.1 &19.2 &0.8 \\
    VideoWorld (Image VQVAE) &Vid &13.8 &20.7 &15.0 &0.5 \\
    VideoWorld &Vid & 56.2 &75.4 &72.1 &45.8 \\
    VideoWorld$^\dagger$ &Vid &\textbf{72.7} &\textbf{91.0} &\textbf{93.8} &\textbf{62.3}\\
% \bottomrule
\end{tabular}
}
\vspace{-1.2em}
\caption{\textbf{CALVIN results.} $\dagger$ denotes using an extra 30k unlabeled data.}
\vspace{-1.5em}
\label{table:re_abla}
\end{table}




% \begin{table} \centering
% \footnotesize
% \scalebox{0.8}{
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{l cc c}
% \toprule[1pt]
%     Data  &Amount &Act-Value &Act-Acc \\
%     \midrule
%     KataGo  \\
%     Human \\
%     Mix  \\
% \bottomrule
% \end{tabular}
% }
% % \vspace{-1.2em}
% \caption{\textbf{Data quality.} }
% \vspace{-1.4em}

% \label{table:idm_data}
% \end{table}


% \begin{table} \centering
% \footnotesize
% \scalebox{0.8}{
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{l cc cc}
% \toprule[1pt]
%     IDM data  &Push &Open/Close &Turn on/off \\
%     \midrule
%     5k  \\
%     10k \\
%     22k  & 56.2 &75.4 &72.1 & \\
% \bottomrule
% \end{tabular}
% }
% % \vspace{-1.2em}
% \caption{\textbf{IDM training set.} }
% \vspace{-1.4em}

% \label{table:data_quality}
% \end{table}

\begin{table}[t]
\centering
\hspace{-2.5em}
%#################################################
% MAE decoder depth
%#################################################
\subfloat[
% Data quality.
Learning with noisy data. 
\label{tab:re_data}
]{
\centering
\begin{minipage}{0.6\linewidth}{\begin{center}
\tablestyle{5pt}{1}
% \vspace{-1em}
\scalebox{0.8}{
% \begin{tabular}{l p{0.7cm} p{1.2cm} p{1cm}}
% \vspace{-em}
\begin{tabular}{p{1.1cm}p{0.4cm} ll}
% \toprule[1pt]
    Data &LDM &Act-Value &Act-Acc \\
    % \midrule
    \specialrule{0em}{0pt}{1pt}
    \shline
    \specialrule{0em}{0pt}{1pt}
    KataGo &\ \ \usym{2717} &\ \ 44.2 &\ \ 41.8\\
    + Human &\ \ \usym{2717} &\ \ 44.7\textcolor{Green}{\tiny{ (+0.5)}} &\ \ 42.2\textcolor{Green}{\tiny{ (+0.4)}}\\
    
    KataGo 
    &\ \ \smash{\raisebox{0.2ex}{\usym{1F5F8}}} &\ \ 67.2 &\ \ 74.9\\
    + Human &\ \ \smash{\raisebox{0.2ex}{\usym{1F5F8}}} &\ \ 69.7\textcolor{Green}{\tiny{ (+2.5)}} &\ \ 76.4\textcolor{Green}{\tiny{ (+1.5)}}\\
% \bottomrule
\end{tabular}
}
\vspace{-0.3em}
\end{center}}
\end{minipage}
}
\hspace{-1.5em}
%#################################################
% MAE decoder width
%#################################################
\subfloat[
Effect of IDM data size.
\label{tab:re_idm}
]{
\begin{minipage}{0.45\linewidth}{\begin{center}
\tablestyle{5pt}{1}
\scalebox{0.8}{
\begin{tabular}{p{0.7cm} p{0.4cm} p{1.1cm} p{1.3cm}}
% \toprule[1pt]
    Amount  &Push &Open/Close &Turn on/off \\
    % \midrule
     \specialrule{0em}{0pt}{1pt}
    \shline
    \specialrule{0em}{0pt}{1pt}
    2k  &\,50.1 &$\quad \ \ $68.8 &$\quad \ \ $67.0\\
    10k & \,54.5 &$\quad \ \ $74.1 &$\quad \ \ $70.3\\
    22k  & \,56.2 &$\quad \ \ $75.4 &$\quad \ \ $72.1 \\
    &&\\
% \bottomrule
\end{tabular}
}
\vspace{-0.5em}
\end{center}}
\end{minipage}
}
\vspace{-0.93em}
\caption{\textbf{More Ablations.}}
\label{tab:re_abla} 
\vspace{-2.2em}
\end{table}

==> tables/re_ablation_v1.tex <==
\vspace{-2em}
\begin{table} \centering
\footnotesize
% \scalebox{0.78}{
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|c|c cc cc}
% \toprule[1pt]
    Method  &Input &Push &Open/Close &Turn on/off &Consecutive \\
    \specialrule{0em}{0pt}{1pt}
    \shline
    \specialrule{0em}{0pt}{1pt}
    SPIL \textcolor{cvprblue}{bit.ly/3CFe4LD} &Vid/Act &68.4&87.9&85.3&55.4 \\
    LCD \textcolor{cvprblue}{bit.ly/3PWna9Q} &Vid/Act &71.3&90.2&92.1&60.7 \\
    {\color{lightgray}Transformer (Oracle)} &{\color{lightgray}Vid/Act} &{\color{lightgray}75.4} &{\color{lightgray}95.3} &{\color{lightgray}96.2} &{\color{lightgray}68.0 }\\
    Transformer &Vid &17.3 &24.1 &19.2 &0.8 \\
    VideoWorld (Img-VQ) &Vid &13.8 &20.7 &15.0 &0.5 \\
    VideoWorld &Vid & 56.2 &75.4 &72.1 &45.8 \\
    VideoWorld$^\dagger$ &Vid &\textbf{72.7} &\textbf{91.0} &\textbf{93.8} &\textbf{62.3}\\
% \bottomrule
\end{tabular}
}
\vspace{-1.3em}
\caption{\textbf{CALVIN results.} $^\dagger$ denotes using an additional 30k data.}
\vspace{-1.5em}
\label{table:re_abla}
\end{table}




% \begin{table} \centering
% \footnotesize
% \scalebox{0.8}{
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{l cc c}
% \toprule[1pt]
%     Data  &Amount &Act-Value &Act-Acc \\
%     \midrule
%     KataGo  \\
%     Human \\
%     Mix  \\
% \bottomrule
% \end{tabular}
% }
% % \vspace{-1.2em}
% \caption{\textbf{Data quality.} }
% \vspace{-1.4em}

% \label{table:idm_data}
% \end{table}


% \begin{table} \centering
% \footnotesize
% \scalebox{0.8}{
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{l cc cc}
% \toprule[1pt]
%     IDM data  &Push &Open/Close &Turn on/off \\
%     \midrule
%     5k  \\
%     10k \\
%     22k  & 56.2 &75.4 &72.1 & \\
% \bottomrule
% \end{tabular}
% }
% % \vspace{-1.2em}
% \caption{\textbf{IDM training set.} }
% \vspace{-1.4em}

% \label{table:data_quality}
% \end{table}

\begin{table}[t]
\centering
\hspace{-2.5em}
%#################################################
% MAE decoder depth
%#################################################
\subfloat[
% Data quality.
Learning with noise data. 
\label{tab:re_data}
]{
\centering
\begin{minipage}{0.6\linewidth}{\begin{center}
\tablestyle{5pt}{1}
\scalebox{0.8}{
% \begin{tabular}{l p{0.7cm} p{1.2cm} p{1cm}}
\begin{tabular}{p{1.1cm}|p{0.5cm}| ll}
% \toprule[1pt]
    Data &LDM &Act-Value &Act-Acc \\
    \specialrule{0em}{0pt}{1pt}
    \shline
    \specialrule{0em}{0pt}{1pt}
    KataGo & &\ \ 44.2 &\ \ 41.8\\
    + Human & &\ \ 44.7\textcolor{Green}{\tiny{ (+0.5)}} &\ \ 42.2\textcolor{Green}{\tiny{ (+0.4)}}\\
    
    KataGo 
    &\ \ \smash{\raisebox{0.2ex}{$\checkmark$}} &\ \ 67.2 &\ \ 74.9\\
    + Human &\ \ \smash{\raisebox{0.2ex}{$\checkmark$}} &\ \ 69.7\textcolor{Green}{\tiny{ (+2.5)}} &\ \ 76.4\textcolor{Green}{\tiny{ (+1.5)}}\\
% \bottomrule
\end{tabular}
}
\vspace{-0.3em}
\end{center}}
\end{minipage}
}
\hspace{-1.5em}
%#################################################
% MAE decoder width
%#################################################
\subfloat[
IDM data.
\label{tab:re_idm}
]{
\begin{minipage}{0.45\linewidth}{\begin{center}
\tablestyle{5pt}{1}
\scalebox{0.8}{
\begin{tabular}{p{0.8cm} p{0.4cm} p{1.1cm} p{1.3cm}}
% \toprule[1pt]
    \multicolumn{1}{l|}{Amount}  &Push &Open/Close &Turn on/off \\
    \specialrule{0em}{0pt}{1pt}
    \shline
    \specialrule{0em}{0pt}{1pt}
    \multicolumn{1}{l|}{2k}  & &\\
    \multicolumn{1}{l|}{10k} & \,54.5 &$\quad \ \ $74.1 &$\quad \ \ $70.3\\
    \multicolumn{1}{l|}{22k}  & \,56.2 &$\quad \ \ $75.4 &$\quad \ \ $72.1 \\
    &&\\
% \bottomrule
\end{tabular}
}
\vspace{-0.3em}
\end{center}}
\end{minipage}
}
\vspace{-1.1em}
\caption{\textbf{More Ablations.}}
\label{tab:data_idm} 
\vspace{-2.2em}
\end{table}

==> tables/supp_baseline.tex <==



\begin{table}[t]
    \footnotesize
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|c|ccc}
        % \toprule
        \multirow{2}*{Methods}   &\multirow{2}*{Input/Ouput} & \multicolumn{3}{c}{Task Success Rate (\%)}\\
        \specialrule{0em}{0pt}{1pt}
        % \cline{3-5}
\specialrule{0em}{0pt}{1pt}
        % \cmidrule(lr){3-5}
        &&Push &Open/Close &Turn on/off\\
        \midrule  
        
        MCIL~\cite{mees2022matterslanguageconditionedrobotic}  &Video/Lab. Action &33.0 &38.7 &41.2 \\
        HULC~\cite{lynch2021languageconditionedimitationlearning}  &Video/Lab. Action &65.8 &80.9 &85.3 \\
        {\color{lightgray}Transformer (Oracle)} &{\color{lightgray}Video/Lab. Action} &{\color{lightgray}75.4} &{\color{lightgray}95.3} &{\color{lightgray}96.2} \\
        Transformer  &Video &17.3 &24.1 &19.2 \\
        \midrule
        Visioner &Video &56.2 &75.4 &72.1 \\
        % \bottomrule            
    \end{tabular}
    }
\caption{\textbf{More comparisons on CALVIN benchmark.} ``Lab.'' means annotated labels. All models have 300M parameters. We additionally compare our results with two open-source works using our testing methods.}  
% \vspace{-1.5em}
\label{table:supp_calvin}
\end{table}

==> tables/table1.tex <==
\begin{center}
\begin{table}[t]
    \footnotesize
       \centering
    % \scalebox{1}
 
        % \begin{footnotesize}
        % \begin{adjustwidth}{2em}{0em}
        % \resizebox{\columnwidth}{!}
        % {
        \begin{tabular}{l|c|c|c}
        % \begin{tabular}{ l|c |@{} ccc | cc c  | c c }
            \toprule
             Input &Video  &Video w/LVPM &State \\
             \specialrule{0em}{0pt}{1pt}
            \hline
            \specialrule{0em}{0pt}{1pt}
             
             % Informativeness & \Checkmark \Checkmark & \Checkmark \Checkmark& \Checkmark \Checkmark &\Checkmark \\
             Informativeness  & $\bigstar$ $\bigstar$ & $\bigstar$ $\bigstar$ &$\bigstar$  \\
             \specialrule{0em}{0pt}{1pt}
             \hline
            compactness& -  & $\bigstar$ &$\bigstar$ $\bigstar$ \\
             
             % \specialrule{0em}{0pt}{1pt}
             % compactness &\XSolidBrush &\Checkmark &\Checkmark &\Checkmark \Checkmark \\
            
            
            \bottomrule            
        \end{tabular}
        % }
        % \end{adjustwidth}
    
        % \end{footnotesize}
    
    \vspace{-1em}
    \caption{}  
    \label{table:table1}   
\vspace{-1em}
\end{table}
\end{center}

==> tables/videog_old.tex <==
\begin{center}
\begin{table*}[t]
    \footnotesize
       \centering
    % \scalebox{1}
 
        % \begin{footnotesize}
        % \begin{adjustwidth}{2em}{0em}
        % \resizebox{2*\columnwidth}{!}
        % {
        % \begin{tabular}{l|c|c|c|c|c|c}
        \begin{tabular}{p{0.1cm}lccccccc}
        % \begin{tabular}{ l|c |@{} ccc | cc c  | c c }
            \toprule
             Idx&Agent &Train &w/o Search &Input &Legal rate (\%) &Action-Value (\%) &Best Action Acc. (\%)  & Tournament Elo\\
             \specialrule{0em}{0pt}{1pt}
            \hline
            \specialrule{0em}{0pt}{1pt}
             
             % Informativeness & \Checkmark \Checkmark & \Checkmark \Checkmark& \Checkmark \Checkmark &\Checkmark \\
             1&KataGO-human-1d  &RL &\XSolidBrush &State &100 &56.8 & 54.2 &2019($\pm$23)  \\

             2&KataGO-human-5d  &RL &\XSolidBrush &State &100 &\underline{70.4} &70.3&2253($\pm$20) \\

             3&{\color{lightgray}KataGO-human-9d (Oracle)}   &{\color{lightgray}RL} &{\color{lightgray}\XSolidBrush} &{\color{lightgray}State} &{\color{lightgray}100} &{\color{lightgray}84.4}&{\color{lightgray}82.0} &{\color{lightgray}2700} \\

            \specialrule{0em}{0pt}{1pt}
            \hline
            \specialrule{0em}{0pt}{1pt}

            4&Transformer 300M  &SL &\Checkmark &State &99.8 &67.0&73.3&2308($\pm$21) \\
            5&Transformer 300M  &SL & \Checkmark &Video&99.6&50.2&49.5&1998($\pm$38) \\

            \specialrule{0em}{0pt}{1pt}
            \hline
            \specialrule{0em}{0pt}{1pt}
            6&Visioner 50M (ours)    &SL & \Checkmark &Video &99.5 &62.1&69.7&2093($\pm$25) \\
            7&Visioner 150M (ours) &SL & \Checkmark &Video &\textbf{99.7} &68.8&74.5&2218($\pm$23) \\
            8&Visioner 300M (ours) &SL & \Checkmark &Video &\textbf{99.7} &\textbf{70.3}&\textbf{78.1}&\textbf{2317}($\pm$25) \\
            
             
            
             % \specialrule{0em}{0pt}{1pt}
             % compactness &\XSolidBrush &\Checkmark &\Checkmark &\Checkmark \Checkmark \\
            
            
            \bottomrule            
        \end{tabular}
        % }
        % \end{adjustwidth}
    
        % \end{footnotesize}
    
    \vspace{-1em}
    \caption{\textbf{Comparison on Video-GoBench.}}  
    \label{table:videogo}   
\vspace{-1em}
\end{table*}
\end{center}
